QCD Structure of Nuclear Interactions

This dissertation investigated selected processes involving baryons and nuclei in hard scattering reactions. Through these processes, this work explored the constituent structure of baryons and the mechanisms through which the interactions between these constituents ultimately control the selected reactions. First, hard nucleon-nucleon elastic scattering was studied considering the quark exchange (QE) between the nucleons to be the dominant mechanism of interaction in the constituent picture. It was found that an angular asymmetry exhibited by proton-neutron (pn) elastic scattering data is explained within this framework if a quark-diquark picture dominates the nucleon's structure instead of a more traditional SU(6) model. The latter yields an asymmetry around 90 deg center of mass scattering with a sign opposite to what is experimentally observed. The second process is the hard breakup by a photon of a nucleon-nucleon system in light nuclei. Proton-proton (pp) and pn breakup in 3He, and double Delta-isobars production in deuteron breakup were analyzed in the hard rescattering model (HRM), which in conjunction with the QE mechanism provides a QCD description of the reaction. Cross sections for both channels in 3He photodisintegration were computed without the need of a fitting parameter. The results presented here for pp breakup show excellent agreement with recent experimental data. In double Delta-isobars production in deuteron breakup, HRM angular distributions for the two double Delta channels were compared to the pn channel and to each other. An important prediction from this study is that the Delta++ Delta- channel consistently dominates Delta+Delta0, which is in contrast with models that unlike the HRM consider a double Delta system in the initial state of the interaction. For such models both channels should have the same strength.

==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 

